Triplet-Watershed for Hyperspectral Image Classification

Hyperspectral images (HSI) consist of rich spatial and spectral information, which can potentially be used for several applications. However, noise, band correlations and high dimensionality restrict the applicability of such data. This is recently addressed using creative deep learning network architectures such as ResNet, SSRN, and A2S2K. However, the last layer, i.e the classification layer, remains unchanged and is taken to be the softmax classifier. In this article, we propose to use a watershed classifier. Watershed classifier extends the watershed operator from Mathematical Morphology for classification. In its vanilla form, the watershed classifier does not have any trainable parameters. In this article, we propose a novel approach to train deep learning networks to obtain representations suitable for the watershed classifier. The watershed classifier exploits the connectivity patterns, a characteristic of HSI datasets, for better inference. We show that exploiting such characteristics allows the Triplet-Watershed to achieve state-of-art results in supervised and semi-supervised contexts. These results are validated on Indianpines (IP), University of Pavia (UP), Kennedy Space Center (KSC) and University of Houston (UH) datasets, relying on simple convnet architecture using a quarter of parameters compared to previous state-of-the-art networks. The source code for reproducing the experiments and supplementary material (high resolution images) is available at https://github.com/ac20/TripletWatershed Code.

==> Table_accuracy_IP.tex <==
\begin{tabular}{ccccccccccc}
    \toprule
        \phantom{abc} & \phantom{abc} & \phantom{abc} &\phantom{abc}& \multicolumn{3}{c}{Classic approaches} & \phantom{abc} & \multicolumn{3}{c}{Deep-Learning approaches}\\
         \cmidrule{5-7}  \cmidrule{9-11}
    Class& Train & Test &\phantom{abc}& RF\cite{IEEE:journals/tgrs/Ham2005} & SVM\cite{DBLP:journals/tgrs/MelganiB04} & Ensemble-Watershed\cite{DBLP:journals/spl/ChallaDSN19} &\phantom{abc}& SSRN\cite{IEEE/journals/tgrs/Zhong2018}& A2S2K\cite{IEEE/journals/tgrs/Roy2020} &Triplet-Watershed\\
    \midrule
                    1 & 4    & 42   &\phantom{abc}& 28.46 $\pm$ 0.061 & 51.22 $\pm$ 0.190 &  41.43 $\pm$ 0.2079 &\phantom{abc}& 57.78 $\pm$ 0.423 & 97.56 $\pm$ 0.034 &\textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray} 2 & 142  & 1286 &\phantom{abc}& 56.63 $\pm$ 0.024 & 81.22 $\pm$ 0.037 &  81.07 $\pm$ 0.0202 &\phantom{abc}& 98.37 $\pm$ 0.012 & 98.62 $\pm$ 0.010 &\textbf{ 99.35 $\pm$ 0.006}\\
                    3 & 83   & 747  &\phantom{abc}& 48.42 $\pm$ 0.013 & 65.82 $\pm$ 0.013 &  71.49 $\pm$ 0.0250 &\phantom{abc}& 97.47 $\pm$ 0.010 & 98.58 $\pm$ 0.006 &\textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray} 4 & 23   & 214  &\phantom{abc}& 33.49 $\pm$ 0.025 & 57.75 $\pm$ 0.041 &  45.70 $\pm$ 0.0327 &\phantom{abc}& 99.12 $\pm$ 0.010 & 98.29 $\pm$ 0.014 &\textbf{100.0 $\pm$ 0.000}\\
                    5 & 48   & 435  &\phantom{abc}& 85.21 $\pm$ 0.025 & 90.04 $\pm$ 0.014 &  92.78 $\pm$ 0.0286 &\phantom{abc}& 97.79 $\pm$ 0.013 & 99.02 $\pm$ 0.003 &\textbf{ 99.17 $\pm$ 0.017}\\
    \rowcolor{Gray} 6 & 73   & 657  &\phantom{abc}& 92.64 $\pm$ 0.027 & 96.25 $\pm$ 0.006 &  98.57 $\pm$ 0.0033 &\phantom{abc}& 98.50 $\pm$ 0.010 & 98.71 $\pm$ 0.010 &\textbf{100.0 $\pm$ 0.000}\\
                    7 & 2    & 26   &\phantom{abc}&  2.67 $\pm$ 0.038 & 73.33 $\pm$ 0.019 &  99.17 $\pm$ 0.0167 &\phantom{abc}& 66.67 $\pm$ 0.471 & 93.10 $\pm$ 0.097 &\textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray} 8 & 47   & 431  &\phantom{abc}& 97.67 $\pm$ 0.015 & 97.98 $\pm$ 0.006 &  98.14 $\pm$ 0.0075 &\phantom{abc}& 96.45 $\pm$ 0.029 & 98.83 $\pm$ 0.016 &\textbf{100.0 $\pm$ 0.000}\\
                    9 & 2    & 18   &\phantom{abc}&  9.26 $\pm$ 0.094 & 50.00 $\pm$ 0.045 &  37.50 $\pm$ 0.1854 &\phantom{abc}& 56.25 $\pm$ 0.418 & 74.26 $\pm$ 0.038 &\textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray} 10 & 97  & 875  &\phantom{abc}& 60.91 $\pm$ 0.047 & 73.87 $\pm$ 0.018 &  85.81 $\pm$ 0.0227 &\phantom{abc}& 98.33 $\pm$ 0.009 & 98.21 $\pm$ 0.016 &\textbf{100.0 $\pm$ 0.000}\\
                    11 & 245 & 2210 &\phantom{abc}& 87.88 $\pm$ 0.019 & 82.90 $\pm$ 0.012 &  86.68 $\pm$ 0.0105 &\phantom{abc}& 99.08 $\pm$ 0.005 & 99.09 $\pm$ 0.001 &\textbf{ 99.42 $\pm$ 0.004}\\
    \rowcolor{Gray} 12 & 59  & 534  &\phantom{abc}& 41.26 $\pm$ 0.030 & 74.91 $\pm$ 0.043 &  69.51 $\pm$ 0.0182 &\phantom{abc}& 98.46 $\pm$ 0.009 & 98.37 $\pm$ 0.013 &\textbf{ 99.06 $\pm$ 0.018}\\
                    13 & 20  & 185  &\phantom{abc}& 90.09 $\pm$ 0.040 & 96.94 $\pm$ 0.021 &  99.35 $\pm$ 0.0079 &\phantom{abc}& 100.0 $\pm$ 0.000 & 99.80 $\pm$ 0.002 &\textbf{100.0 $\pm$ 0.000} \\
    \rowcolor{Gray} 14 & 126 & 1139 &\phantom{abc}& 95.46 $\pm$ 0.014 & 93.82 $\pm$ 0.010 &  92.59 $\pm$ 0.0085 &\phantom{abc}& 98.63 $\pm$ 0.010 & 99.22 $\pm$ 0.007 &\textbf{100.0 $\pm$ 0.000} \\
                    15 & 38  & 348  &\phantom{abc}& 41.11 $\pm$ 0.029 & 60.42 $\pm$ 0.044 &  54.48 $\pm$ 0.0396 &\phantom{abc}& 99.24 $\pm$ 0.005 & 97.86 $\pm$ 0.013 &\textbf{100.0 $\pm$ 0.000} \\
    \rowcolor{Gray} 16 & 9   & 84   &\phantom{abc}& 79.37 $\pm$ 0.030 & 91.27 $\pm$ 0.054 &  79.29 $\pm$ 0.1163 &\phantom{abc}& 95.63 $\pm$ 0.062 & 95.93 $\pm$ 0.057 &\textbf{ 98.10 $\pm$ 0.033}\\
    \midrule
                    OA & 1018 & 9231 &\phantom{abc}& 72.98 $\pm$ 0.006  & 82.00 $\pm$ 0.006  & 83.75 $\pm$ 0.0076  &\phantom{abc}& 98.38 $\pm$ 0.004  & 98.66 $\pm$ 0.004& \textbf{99.66  $\pm$ 0.002} \\
    \rowcolor{Gray} AA &      &      &\phantom{abc}& 59.41 $\pm$ 0.005  & 77.36 $\pm$ 0.019  & 77.10 $\pm$ 0.0228  &\phantom{abc}& 91.11 $\pm$ 0.080  & 96.59 $\pm$ 0.003& \textbf{99.69  $\pm$ 0.002} \\
    $\kappa$ &&      &\phantom{abc}& 0.6862 $\pm$ 0.007 & 0.7941 $\pm$ 0.007 & 0.8143 $\pm$ 0.0086  &\phantom{abc}& 0.9815 $\pm$ 0.005 & 0.9848 $\pm$ 0.005& \textbf{0.9961 $\pm$ 0.002} \\
    \bottomrule
    \end{tabular}

==> Table_accuracy_IP_semisupervised.tex <==
\begin{tabular}{ccccccccc}
\toprule
Class& Train & Test &\phantom{abc}& S2GCN\cite{IEEE:journal/grsl/Qin2019} & SSRN\cite{IEEE/journals/tgrs/Zhong2018} & DC-GCN\cite{ARXIV:Zeng2020} &  Triplet-Watershed\\
\midrule
                1  & 30 & 16   &\phantom{abc}&   \textbf{100.0 $\pm$ 0.0000} &   93.24 $\pm$ 0.0263 &  \textbf{100.00 $\pm$  0.0000} &  \textbf{100.00 $\pm$ 0.0000}  \\
\rowcolor{Gray} 2  & 30 & 1398 &\phantom{abc}&    84.43 $\pm$ 0.0250 &   76.63 $\pm$ 0.0596 &   91.28 $\pm$  0.0360 &   \textbf{96.59 $\pm$ 0.0194}  \\
                3  & 30 & 800  &\phantom{abc}&    82.87 $\pm$ 0.0553 &   68.78 $\pm$ 0.0753 &   92.88 $\pm$  0.0396 &  \textbf{100.00 $\pm$ 0.0000}  \\
\rowcolor{Gray} 4  & 30 & 207  &\phantom{abc}&    93.08 $\pm$ 0.0195 &   87.64 $\pm$ 0.0249 &   98.11 $\pm$  0.0151 &  \textbf{100.00 $\pm$ 0.0000}  \\
                5  & 30 & 453  &\phantom{abc}&    97.13 $\pm$ 0.0134 &   86.72 $\pm$ 0.0154 &   95.54 $\pm$  0.0339 &   \textbf{99.20 $\pm$ 0.0158}  \\
\rowcolor{Gray} 6  & 30 & 700  &\phantom{abc}&    97.29 $\pm$ 0.0127 &   92.05 $\pm$ 0.0182 &   98.67 $\pm$  0.0104 &  \textbf{100.00 $\pm$ 0.0000}  \\
                7  & 15 & 13   &\phantom{abc}&    92.31 $\pm$ 0.0000 &   95.66 $\pm$ 0.0051 &  \textbf{100.00 $\pm$  0.0000} &  \textbf{100.00 $\pm$ 0.0000}  \\
\rowcolor{Gray} 8  & 30 & 448  &\phantom{abc}&    99.03 $\pm$ 0.0093 &   95.90 $\pm$ 0.0297 &  \textbf{100.00 $\pm$  0.0000} &  \textbf{100.00 $\pm$ 0.0000}  \\
                9  & 15 & 5    &\phantom{abc}&   \textbf{100.00 $\pm$ 0.0000} &  \textbf{100.00 $\pm$ 0.0000} &  \textbf{100.00 $\pm$  0.0000} &  \textbf{100.00 $\pm$ 0.0000}  \\
\rowcolor{Gray} 10 & 30 & 942  &\phantom{abc}&    93.77 $\pm$ 0.0373 &   82.42 $\pm$ 0.0324 &   91.91 $\pm$  0.0378 &   \textbf{99.10 $\pm$ 0.0114}  \\
                11 & 30 & 2425 &\phantom{abc}&    84.98 $\pm$ 0.0282 &   82.23 $\pm$ 0.0288 &   91.79 $\pm$  0.0379 &   \textbf{97.01 $\pm$ 0.0296}  \\
\rowcolor{Gray} 12 & 30 & 563  &\phantom{abc}&    80.05 $\pm$ 0.0517 &   69.09 $\pm$ 0.0436 &   90.17 $\pm$  0.0554 &   \textbf{98.93 $\pm$ 0.0116}  \\
                13 & 30 & 175  &\phantom{abc}&    99.43 $\pm$ 0.0000 &   95.78 $\pm$ 0.0075 &   99.65 $\pm$  0.0027 &  \textbf{100.00 $\pm$ 0.0000}  \\
\rowcolor{Gray} 14 & 30 & 1235 &\phantom{abc}&    96.73 $\pm$ 0.0092 &   86.52 $\pm$ 0.0243 &   99.73 $\pm$  0.0066 &  \textbf{100.00 $\pm$ 0.0000}  \\
                15 & 30 & 356  &\phantom{abc}&    86.80 $\pm$ 0.0342 &   73.12 $\pm$ 0.0528 &   99.94 $\pm$  0.0016 &  \textbf{100.00 $\pm$ 0.0000}  \\
\rowcolor{Gray} 16 & 30 & 63   &\phantom{abc}&   \textbf{100.00 $\pm$ 0.0000} &   86.21 $\pm$ 0.0130 &  \textbf{100.00 $\pm$  0.0000} &   99.36 $\pm$ 0.0077  \\
\midrule
                OA &      &      &\phantom{abc}&  89.4 $\pm$ 0.0108  &  88.34 $\pm$ 0.0173 &   94.65 $\pm$  0.1210 &   \textbf{98.58 $\pm$ 0.0090}   \\
\rowcolor{Gray} AA &      &      &\phantom{abc}&  92.9 $\pm$ 0.0104  &  85.75 $\pm$ 0.0069 &   96.85 $\pm$  0.0040 &   \textbf{99.39 $\pm$ 0.0033}   \\
          $\kappa$ &      &      &\phantom{abc}& 0.880 $\pm$ 0.012   & 0.866  $\pm$ 0.019  & 0.944   $\pm$  0.014  &  \textbf{0.983 $\pm$ 0.010}  \\
\bottomrule
\end{tabular}

==> Table_accuracy_KSC.tex <==
\begin{tabular}{ccccccccccc}

    \toprule
    \phantom{abc} & \phantom{abc} & \phantom{abc} &\phantom{abc}& \multicolumn{3}{c}{Classic approaches} & \phantom{abc} & \multicolumn{3}{c}{Deep-Learning approaches}\\
         \cmidrule{5-7}  \cmidrule{9-11}
    Class& Train & Test &\phantom{abc}& RF\cite{IEEE:journals/tgrs/Ham2005} & SVM\cite{DBLP:journals/tgrs/MelganiB04} & Ensemble-Watershed\cite{DBLP:journals/spl/ChallaDSN19} &\phantom{abc}& SSRN\cite{IEEE/journals/tgrs/Zhong2018}& A2S2K\cite{IEEE/journals/tgrs/Roy2020} & Triplet-Watershed\\
    \midrule
                   1 & 76 & 685 &\phantom{abc}& 94.79 $\pm$ 0.012 & 95.43 $\pm$ 0.023 &  96.23 $\pm$ 0.0085 &\phantom{abc}& 99.95 $\pm$ 0.001 & 99.95  $\pm$ 0.001                           &  \textbf{100.0 $\pm$ 0.0000}\\
    \rowcolor{Gray}2 & 24 & 219 &\phantom{abc}& 81.58 $\pm$ 0 047 & 83.71 $\pm$ 0.012 &  89.59 $\pm$ 0.0247 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & 98.68  $\pm$ 0.019                  &  \textbf{100.0 $\pm$ 0.0000}\\
                   3 & 25 & 231 &\phantom{abc}& 86.09 $\pm$ 0 020 & 78.41 $\pm$ 0.218 &  83.98 $\pm$ 0.0341 &\phantom{abc}& 99.66 $\pm$ 0.005 & 98.72  $\pm$ 0.012                           &  \textbf{100.0 $\pm$ 0.0000}\\
    \rowcolor{Gray}4 & 25 & 227 &\phantom{abc}& 71.22 $\pm$ 0.061 & 27.17 $\pm$ 0.173 &  69.60 $\pm$ 0.0406 &\phantom{abc}& 91.22 $\pm$ 0.047 & 94.27  $\pm$ 0.042                           &  \textbf{97.00 $\pm$ 0.0356}\\
                   5 & 16 & 145 &\phantom{abc}& 47.59 $\pm$ 0.060 & 22.99 $\pm$ 0.170 &  65.52 $\pm$ 0.0474 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & 94.46  $\pm$ 0.050                  &  98.07 $\pm$ 0.0252\\
    \rowcolor{Gray}6 & 22 & 207 &\phantom{abc}& 48.22 $\pm$ 0.014 & 36.89 $\pm$ 0.078 &  53.33 $\pm$ 0.0526 &\phantom{abc}& 98.45 $\pm$ 0.022 & 99.82  $\pm$ 0.003                           &  \textbf{98.84 $\pm$ 0.0135}\\
                   7 & 10 & 95  &\phantom{abc}& 79.43 $\pm$ 0 096 & 87.94 $\pm$ 0.027 &  85.05 $\pm$ 0.0234 &\phantom{abc}& 95.42 $\pm$ 0.050 & 99.61  $\pm$ 0.005                           &  \textbf{100.0 $\pm$ 0.0000}\\
    \rowcolor{Gray}8 & 43 & 388 &\phantom{abc}& 78.61 $\pm$ 0.054 & 70.19 $\pm$ 0.073 &  91.24 $\pm$ 0.0297 &\phantom{abc}& 99.80 $\pm$ 0.003 & \textbf{100.0  $\pm$ 0.000}                  &  \textbf{100.0 $\pm$ 0.0000}\\
                   9 & 52 & 468 &\phantom{abc}& 89.46 $\pm$ 0.011 & 85.33 $\pm$ 0.021 &  93.08 $\pm$ 0.0193 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & \textbf{100.0  $\pm$ 0.000}         &  \textbf{100.0 $\pm$ 0.0000}\\
    \rowcolor{Gray}10 &40 & 364 &\phantom{abc}& 88.43 $\pm$ 0.034 & 78.88 $\pm$ 0.069 &  92.64 $\pm$ 0.0150 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & \textbf{100.0  $\pm$ 0.000}         &  \textbf{100.0 $\pm$ 0.0000}\\
                   11 &41 & 378 &\phantom{abc}& 95.58 $\pm$ 0.014 & 93.81 $\pm$ 0.008 &  94.44 $\pm$ 0.0261 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & \textbf{100.0  $\pm$ 0.000}         &  \textbf{100.0 $\pm$ 0.0000}\\
    \rowcolor{Gray}12 &50 & 453 &\phantom{abc}& 82.63 $\pm$ 0.032 & 86.98 $\pm$ 0.009 &  86.98 $\pm$ 0.0119 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & \textbf{100.0  $\pm$ 0.000}         & 98.28 $\pm$ 0.0212\\
                   13 &92 & 835 &\phantom{abc}& 99.60 $\pm$ 0.002 & \textbf{100.0 $\pm$ 0.000} &  99.69 $\pm$ 0.0022 &\phantom{abc}& \textbf{100.0 $\pm$ 0.000} & \textbf{100.0  $\pm$ 0.000}&  \textbf{100.0 $\pm$ 0.0000} \\
    \midrule
                   OA & 516 & 4695  &\phantom{abc}& 86.17  $\pm$ 0.004  & 81.27 $\pm$ 0.008   & 89.54 $\pm$ 0.0038 &\phantom{abc}& 99.29 $\pm$ 0.004   & 99.34 $\pm$ 0.0008 & \textbf{99.58  $\pm$ 0.0031}\\
    \rowcolor{Gray}AA &      &      &\phantom{abc}& 80.25  $\pm$ 0.004  & 72.90 $\pm$ 0.021   & 84.72 $\pm$ 0.0038 &\phantom{abc}& 98.80 $\pm$ 0.008   & 98.88 $\pm$ 0.0018 & \textbf{99.40  $\pm$ 0.0045}\\
    $\kappa$ &&      &\phantom{abc}& 0.8459 $\pm$ 0.004  & 0.7909 $\pm$ 0.009  & 0.8834 $\pm$ 0.0042 &\phantom{abc}& 0.9921 $\pm$ 0.004  & 0.9927 $\pm$ 0.001 & \textbf{0.9953 $\pm$ 0.0035}\\
    \bottomrule
    \end{tabular}


==> Table_accuracy_UP.tex <==
\begin{tabular}{ccccccccccc}
    \toprule
        \phantom{abc} & \phantom{abc} & \phantom{abc} &\phantom{abc}& \multicolumn{3}{c}{Classic approaches} & \phantom{abc} & \multicolumn{3}{c}{Deep-Learning approaches}\\
                 \cmidrule{5-7}  \cmidrule{9-11}
    Class& Train & Test &\phantom{abc}& RF\cite{IEEE:journals/tgrs/Ham2005} & SVM\cite{DBLP:journals/tgrs/MelganiB04} & Ensemble-Watershed\cite{DBLP:journals/spl/ChallaDSN19} &\phantom{abc}& SSRN\cite{IEEE/journals/tgrs/Zhong2018}& A2S2K\cite{IEEE/journals/tgrs/Roy2020} & Triplet-Watershed\\
    \midrule
                   1  & 663  & 5968   &\phantom{abc}& 91.11 $\pm$ 0.007   & 94.30  $\pm$ 0.008  & 94.34 $\pm$ 0.0032 &\phantom{abc}& 99.85  $\pm$ 0.001           & 99.91  $\pm$ 0.000          & \textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray}2  & 1864 & 16785  &\phantom{abc}& 98.11 $\pm$ 0.003   & 97.65  $\pm$ 0.002  & 95.24 $\pm$ 0.0051 &\phantom{abc}& 99.98  $\pm$ 0.000           & 99.99  $\pm$ 0.000          & \textbf{100.0 $\pm$ 0.000}\\
                   3  & 209  & 1890   &\phantom{abc}& 67.71 $\pm$ 0.014   & 81.26  $\pm$ 0.018  & 69.39 $\pm$ 0.0151 &\phantom{abc}& 99.68  $\pm$ 0.003           & 99.88  $\pm$ 0.001          & \textbf{99.82 $\pm$ 0.004}\\
    \rowcolor{Gray}4  & 306  & 2758   &\phantom{abc}& 88.20 $\pm$ 0.006   & 94.63  $\pm$ 0.004  & 78.69 $\pm$ 0.0058 &\phantom{abc}& 99.92  $\pm$ 0.001           & 99.95  $\pm$ 0.001          & \textbf{99.99 $\pm$ 0.001}\\
                   5  & 134  & 1211   &\phantom{abc}& 98.93 $\pm$ 0.002   & 99.20  $\pm$ 0.002  & 87.46 $\pm$ 0.0110 &\phantom{abc}& 99.94  $\pm$ 0.000           & \textbf{100.0  $\pm$ 0.000} & \textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray}6  & 502  & 4527   &\phantom{abc}& 72.14 $\pm$ 0,022   & 90.58  $\pm$ 0,008  & 61.37 $\pm$ 0.0111 &\phantom{abc}& 99.95  $\pm$ 0.001           & 99.91  $\pm$ 0,001          & \textbf{100.0 $\pm$ 0.000}\\
                   7  & 133  & 1197   &\phantom{abc}& 75.69 $\pm$ 0.017   & 85.71  $\pm$ 0.011  & 75.49 $\pm$ 0.0295 &\phantom{abc}& \textbf{100.0  $\pm$ 0.000}  & \textbf{100.0  $\pm$ 0.000} & \textbf{100.0 $\pm$ 0.000}\\
    \rowcolor{Gray}8  & 368  & 3314   &\phantom{abc}& 89.64 $\pm$ 0.013   & 88.20  $\pm$ 0.003  & 74.65 $\pm$ 0.0044 &\phantom{abc}& 98.28  $\pm$ 0.015           & 98.88  $\pm$ 0.006          & \textbf{99.99 $\pm$ 0.001}\\
                   9  & 94   & 853    &\phantom{abc}& 99.77 $\pm$ 0.002   & 99.84  $\pm$ 0.001  & 99.77 $\pm$ 0.0015 &\phantom{abc}& 99.39  $\pm$ 0.003           & 99.78  $\pm$ 0.003          & \textbf{100.0 $\pm$ 0.000}\\
    \midrule
                   OA &4273  & 38503  &\phantom{abc}& 90.41 $\pm$ 0.001   & 94.19  $\pm$ 0.002  & 86.13 $\pm$ 0.0023 &\phantom{abc}& 99.77  $\pm$ 0.001  & 99.85  $\pm$ 0.001 & \textbf{99.99 $\pm$ 0.002}  \\
    \rowcolor{Gray}AA &      &        &\phantom{abc}& 86.81 $\pm$ 0.002   & 92.38  $\pm$ 0.003  & 81.82 $\pm$ 0.0039&\phantom{abc}& 99.66  $\pm$ 0.001  & 99.81  $\pm$ 0.001 &\textbf{99.98 $\pm$ 0.004} \\
    $\kappa$ &&        &\phantom{abc}& 0.8710 $\pm$ 0.002  & 0.9229 $\pm$ 0.002  & 0.8136 $\pm$ 0.0030 &\phantom{abc}& 0.9969 $\pm$ 0.001  & 0.9981 $\pm$ 0.001 & \textbf{0.9999 $\pm$ 0.002} \\    \bottomrule
    \end{tabular}

==> Table_accuracy_UP_semisupervised.tex <==
\begin{tabular}{ccccccccc|}
\toprule
Class& Train & Test &\phantom{abc}& S2GCN\cite{IEEE:journal/grsl/Qin2019} & SSRN\cite{IEEE/journals/tgrs/Zhong2018} & DC-GCN\cite{ARXIV:Zeng2020} &  Triplet-Watershed\\
\midrule
                1  & 30  & 6601    &\phantom{abc}&   92.78 $\pm$ 0.0379   &  98.80 $\pm$ 0.0110  &  92.85 $\pm$ 0.0351   &   \textbf{99.20   $\pm$ 0.0148}  \\
\rowcolor{Gray} 2  & 30  & 18619   &\phantom{abc}&   87.06 $\pm$ 0.0447   &  98.45 $\pm$ 0.0054  &  97.53 $\pm$ 0.0140   &  \textbf{100.00   $\pm$ 0.0000}  \\
                3  & 30  & 2069    &\phantom{abc}&   87.97 $\pm$ 0.0477   &  77.05 $\pm$ 0.1024  &  97.94 $\pm$ 0.0118   &   \textbf{99.83   $\pm$ 0.0032}  \\
\rowcolor{Gray} 4  & 30  & 3034    &\phantom{abc}&   90.85 $\pm$ 0.0094   &  83.02 $\pm$ 0.0907  &  94.57 $\pm$ 0.0109   &   \textbf{99.98   $\pm$ 0.0002}  \\
                5  & 30  & 1315    &\phantom{abc}&  \textbf{100.00 $\pm$ 0.0000}   &  99.96 $\pm$ 0.0009  &  99.49 $\pm$ 0.0068   &  \textbf{100.00   $\pm$ 0.0000}  \\
\rowcolor{Gray} 6  & 30  & 4999    &\phantom{abc}&   88.69 $\pm$ 0.0264   &  87.03 $\pm$ 0.0626  &  98.57 $\pm$ 0.0278   &   \textbf{99.99   $\pm$ 0.0001}  \\
                7  & 30  & 1300    &\phantom{abc}&   98.88 $\pm$ 0.0108   &  83.92 $\pm$ 0.0897  & \textbf{100.00 $\pm$ 0.0000}   &  \textbf{100.00   $\pm$ 0.0000}  \\
\rowcolor{Gray} 8  & 30  & 3652    &\phantom{abc}&   89.97 $\pm$ 0.0328   &  88.41 $\pm$ 0.0463  &  \textbf{96.00 $\pm$ 0.0277}   &   87.42   $\pm$ 0.1380  \\
                9  & 30  & 917     &\phantom{abc}&   98.89 $\pm$ 0.0053   &  99.97 $\pm$ 0.0004  &  97.51 $\pm$ 0.0140   &  \textbf{100.00   $\pm$ 0.0000}  \\
\midrule
                OA &      &        &\phantom{abc}&   89.74 $\pm$ 0.0170   &  92.81 $\pm$ 0.0190  &  96.87 $\pm$ 0.0111   &   \textbf{98.78   $\pm$ 0.0118} \\
\rowcolor{Gray} AA &      &        &\phantom{abc}&   92.80 $\pm$ 0.0047   &  90.73 $\pm$ 0.0226  &  97.16 $\pm$ 0.0076   &   \textbf{98.49   $\pm$ 0.0151} \\
                $\kappa$ &&        &\phantom{abc}&  0.8665 $\pm$ 0.020    & 0.9059 $\pm$ 0.024   & 0.9677 $\pm$ 0.012    &   \textbf{0.9830  $\pm$ 0.015} \\
\bottomrule
\end{tabular}

==> Table_number_comp.tex <==
\begin{tabular}{cccccccc}
    \toprule
     \multicolumn{2}{c}{IP} & \phantom{abc} & \multicolumn{2}{c}{UP} & \phantom{abc} & \multicolumn{2}{c}{KSC} \\
    Label & Component & \phantom{abc} & Label & Component & \phantom{abc} &Label & Component \\
    \midrule
                  1           &46           &\phantom{abc} &1             &6631          &\phantom{abc} &1              &761           \\
\rowcolor{Gray}   2           &1428         &\phantom{abc} &2             &18649         &\phantom{abc} &2              &243           \\
                  3           &830          &\phantom{abc} &3             &2099          &\phantom{abc} &3              &256           \\
\rowcolor{Gray}   4           &237          &\phantom{abc} &4             &3064          &\phantom{abc} &4              &252           \\
                  5           &147, 318, 18 &\phantom{abc} &5             &1345          &\phantom{abc} &5              &161           \\
\rowcolor{Gray}   6           &730          &\phantom{abc} &6             &5029          &\phantom{abc} &6              &228,1         \\
                  7           &28           &\phantom{abc} &7             &1330          &\phantom{abc} &7              &105           \\
\rowcolor{Gray}   8           &478          &\phantom{abc} &8             &3682          &\phantom{abc} &8              &431           \\
                  9           &20           &\phantom{abc} &9             &947           &\phantom{abc} &9              &520           \\
\rowcolor{Gray}   10          &912, 60      &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &10             &404           \\
                  11          &2455         &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &11             &419           \\
\rowcolor{Gray}   12          &593          &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &12             &503           \\
                  13          &205          &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &13             &927           \\
\rowcolor{Gray}   14          &1265         &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc}  &\phantom{abc} \\
                  15          &386          &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc}  &\phantom{abc} \\
\rowcolor{Gray}   16          &93           &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc} &\phantom{abc}  &\phantom{abc} \\
\bottomrule
\end{tabular}



